Unavoidable patterns in locally balanced colourings

Which patterns must a two-colouring of $K_n$ contain if each vertex has at least $\varepsilon n$ red and $\varepsilon n$ blue neighbours? In this paper, we investigate this question and its multicolour variant. For instance, we show that any such graph contains a $t$-blow-up of an \textit{alternating 4-cycle} with $t = \Omega(\log n)$.

==> tikz-3-colours-srccode.tex <==
%26 august 2022

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,305); %set diagram left start at 0, and has height of 305

%Straight Lines [id:da5300502861572356] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=6]    (225,105) -- (315,45) ;
%Straight Lines [id:da9752487311039989] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=6]    (405,195) -- (405,105) ;
%Straight Lines [id:da08832123284171578] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=6]    (315,255) -- (225,195) ;
%Straight Lines [id:da8914386812069515] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=6]    (315,45) -- (405,105) ;
%Straight Lines [id:da2209795335194158] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=6]    (315,255) -- (405,195) ;
%Straight Lines [id:da41436501070816123] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=6]    (225,195) -- (225,105) ;
%Straight Lines [id:da8016499800365835] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=6]    (315,255) -- (315,45) ;
%Straight Lines [id:da23538488922274037] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=6]    (405,105) -- (225,105) ;
%Straight Lines [id:da00411785915064955] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=6]    (405,195) -- (225,195) ;
%Straight Lines [id:da9503523735341298] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=6]    (315,45) -- (225,195) ;
%Straight Lines [id:da46362353812619594] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=6]    (225,105) -- (315,255) ;
%Straight Lines [id:da5887073630116666] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=6]    (405,105) -- (315,255) ;
%Straight Lines [id:da8555185107228656] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=6]    (225,195) -- (405,105) ;
%Straight Lines [id:da6867845661495712] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=6]    (315,45) -- (405,195) ;
%Straight Lines [id:da1356752228475967] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=6]    (225,105) -- (405,195) ;
%Shape: Ellipse [id:dp9133702279885019] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (300,45) .. controls (300,36.72) and (306.72,30) .. (315,30) .. controls (323.28,30) and (330,36.72) .. (330,45) .. controls (330,53.28) and (323.28,60) .. (315,60) .. controls (306.72,60) and (300,53.28) .. (300,45) -- cycle ;
%Shape: Ellipse [id:dp4286059305621669] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (390,105) .. controls (390,96.72) and (396.72,90) .. (405,90) .. controls (413.28,90) and (420,96.72) .. (420,105) .. controls (420,113.28) and (413.28,120) .. (405,120) .. controls (396.72,120) and (390,113.28) .. (390,105) -- cycle ;
%Shape: Ellipse [id:dp5625762415114526] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (390,195) .. controls (390,186.72) and (396.72,180) .. (405,180) .. controls (413.28,180) and (420,186.72) .. (420,195) .. controls (420,203.28) and (413.28,210) .. (405,210) .. controls (396.72,210) and (390,203.28) .. (390,195) -- cycle ;
%Shape: Ellipse [id:dp7314850934516922] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (300,255) .. controls (300,246.72) and (306.72,240) .. (315,240) .. controls (323.28,240) and (330,246.72) .. (330,255) .. controls (330,263.28) and (323.28,270) .. (315,270) .. controls (306.72,270) and (300,263.28) .. (300,255) -- cycle ;
%Shape: Ellipse [id:dp30854572804755453] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (210,195) .. controls (210,186.72) and (216.72,180) .. (225,180) .. controls (233.28,180) and (240,186.72) .. (240,195) .. controls (240,203.28) and (233.28,210) .. (225,210) .. controls (216.72,210) and (210,203.28) .. (210,195) -- cycle ;
%Shape: Ellipse [id:dp11778987180021583] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (210,105) .. controls (210,96.72) and (216.72,90) .. (225,90) .. controls (233.28,90) and (240,96.72) .. (240,105) .. controls (240,113.28) and (233.28,120) .. (225,120) .. controls (216.72,120) and (210,113.28) .. (210,105) -- cycle ;




\end{tikzpicture}

